Sharp Multiple Instance Learning for DeepFake Video Detection

With the rapid development of facial manipulation techniques, face forgery has received considerable attention in multimedia and computer vision community due to security concerns. Existing methods are mostly designed for single-frame detection trained with precise image-level labels or for video-level prediction by only modeling the inter-frame inconsistency, leaving potential high risks for DeepFake attackers. In this paper, we introduce a new problem of partial face attack in DeepFake video, where only video-level labels are provided but not all the faces in the fake videos are manipulated. We address this problem by multiple instance learning framework, treating faces and input video as instances and bag respectively. A sharp MIL (S-MIL) is proposed which builds direct mapping from instance embeddings to bag prediction, rather than from instance embeddings to instance prediction and then to bag prediction in traditional MIL. Theoretical analysis proves that the gradient vanishing in traditional MIL is relieved in S-MIL. To generate instances that can accurately incorporate the partially manipulated faces, spatial-temporal encoded instance is designed to fully model the intra-frame and inter-frame inconsistency, which further helps to promote the detection performance. We also construct a new dataset FFPMS for partially attacked DeepFake video detection, which can benefit the evaluation of different methods at both frame and video levels. Experiments on FFPMS and the widely used DFDC dataset verify that S-MIL is superior to other counterparts for partially attacked DeepFake video detection. In addition, S-MIL can also be adapted to traditional DeepFake image detection tasks and achieve state-of-the-art performance on single-frame datasets.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> intro.tex <==
The rise of face manipulation techniques \cite{DeepFakes,FaceSwap,Justus2018Face2Face,Deferred} has fueled the advent of forgery face images and videos. In the beginning, theses tools are only used to create face swaps videos for fun. However, when the swapped faces become more and more believable, these techniques are abused for malicious purposes, even for political persecution or face recognition attack. Thus, it is vital to develop more advanced detection technology.

Most existing works \cite{DingSwapped,Shahroz,Marra2018Detection,Faceforensics,Faceforensics++} detect forgery from frames with face manipulation individually. For such forgery faces, these detection methods work quite well and reach around 98\% detection accuracy. However, when the scenario transforms into a video with multiple instances, the performance of them drops a lot. In a multiple instance learning (MIL) task, a video that contains one fake frame should be judged as fake. Figure 1 shows forgery face detection examples for four nearby frames from a video. It illustrates that multiple faces may appear in the same frame and an identical person may have real or fake faces in nearby frames. In some frames, neither face has been tampered.

The existing methods have several difficulties when facing MIL forgery face detection. Firstly, these methods tend to sample frames from a video. Unless they recognize every frame in the video, which is very resource consuming, otherwise, these methods may miss frames that have been tampered. For instance, if they only sample the frames like `Frame 40th' without tampered face, the prediction result of this video will be `real'. Thus, the traditional methods for single-frame detection are restricted in practical application, which leaves a potential risk for deepfake attackers. Secondly, the typical face forgery method like Deepfake \cite{DeepFakes} usually tampers the video by single-frame, which may cause some jitter in the nearby frames. But the existing single-frame level methods are not sensitive enough to these jitters, which wastes a vital clue of fake video. In addition, for existing face forgery detection task, the training data needs to label every image with real or fake annotation. For a 60 seconds deepfake video, previous methods \cite{X-ray,Guera} typically require more than 30 frames with labels. On the contrary, our MIL approach only requires a real or fake label for the video, which is much more convenient. Therefore, due to the above limitations, the existing methods can no longer satisfy the needs of forgery face recognition.

In this paper, we introduce a novel problem of multi-instance face forgery detection and propose a novel network named Sharp Multi-Instance Learning Net (S-MIL Net) driven by a weighting mechanism. We design the network as a multi-scale architecture composed of a spatial-level encoding part and a temporal-level encoding part, which can learn local frame feature and nearby frame features, respectively. Given a video sequence, our approach can predict real or fake by considering the semantics among nearby frames rather than the max or mean score of several frames, which is more sensitive to the jitter. On the other hand, the proposed weighting mechanism relieves the vanishing gradients issue which commonly appears in the Multi-Instance learning task. In a MIL task, the key problem is the learning process from instance decision to bag level decision. The traditional method achieve the bag level decision without focus, which may cause gradients vanishing during the training. In our approach, the weighting mechanism is utilized to enhance the weights of important frames while weaken the irrelevant ones, which visually makes the gradient surface much sharper. 

Besides, we propose a new dataset named FaceForensics Plus with Mixing samples (FFPMS) for multi-instance detection, which only requires video-level label. We believe that this dataset can inspire more video-level methods and push the forgery detection field to a new level. Experiments on our FFPMS dataset verify that our approach is superior to other counterparts for multi-instance face forgery detection. Also, the proposed method can make a more accurate judge on whether a video is fake or not than other methods on DFDC benchmark. Moreover, our S-MIL Net can also be adapted to traditional single-frame detection task and achieves SOTA performance on the FF++ datasets \cite{Faceforensics++}, showing a promising result for face information protection. 



The major contributions of our paper include: 

\begin{itemize}
\item We introduce a novel framework for multi-instance face forgery detection and a new FFPMS dataset with video-level annotation, which is more close to the practical application.

\item We propose a multi-scale network named S-MIL Net driven by a weighting mechanism, which can learn semantics among nearby frames and relieve the vanishing gradients issue as well.

\item We verify that our approach is superior to other counterparts for multi-instance face forgery detection and our S-MIL Net can also be adapted to traditional single-frame detection.
\end{itemize}


==> intro1.tex <==
The rise of face manipulation techniques has fueled the advent of forgery face images and videos~\cite{DeepFakes,FaceSwap,Justus2018Face2Face,Deferred}. In early years, these tools were only used to create face swaps videos for entertainment. However, when the swapped faces become more and more lifelike with advanced deep learning models such as Generative Adversarial Networks (GAN), these techniques, {\it e.g.}, DeepFake~\cite{DeepFakes}, are abused for malicious purposes, {\it e.g.}, face recognition attack or even political persecution. To enhance the content security,
it is crucial to develop more advanced forgery image and video detection technology.

Most existing works~\cite{DingSwapped,Shahroz,Marra2018Detection,Faceforensics,Faceforensics++} detect face manipulation in a frame-by-frame fashion. These frame-based detection methods work quite well and reach a high detection accuracy up to 98\%. However, when the application scenario is transferred into video domains, their performance drops significantly due to the lack of frame-level forgery annotation.
Generally, a video that contains even a fake face in one single frame should be judged as fake. The challenge and difficulty of video forgery detection is illustrated by the example of forgery faces on four nearby frames from a video in Fig.~\ref{fig:teaser}. We see that multiple faces may appear in the same frame. One person may have real or fake faces in nearby frames, while in some frames, neither face has been manipulated. More importantly, the manipulated fake faces looks highly similar to the real faces, which makes the video forgery detection task even harder.


Existing frame-based methods meet with several difficulties when applied to video forgery face detection. First, frame-based models are generally data hungry which requires a remarkable amount of labeled frames for training~\cite{X-ray,Guera}.
Furthermore, during the inference stage, every frame in the video have to be processed to produce frame-level prediction, which is very computationally exhaustive. Sampling part of frames will lead to the missing of manipulated frames. For instance, if only the 40th frame without tampered face is sampled in Figure 1, the forgery detection result of this video will be `real'.
Thus, traditional frame-based methods are restricted in practical application, which leaves potential risks for deepfake attackers. 

%For example, for a 60-second video, previous methods  typically require more than 30 frames to be annotated.

To address the video fogery detection problem by using only video level annotation, we put forward a new learning framework based on Multiple Instance Learning framework (MIL). Generally, each face, regardless of real or fake, can be treated as an instance, and all the faces of a video can be treated as a bag of instances. Annotating a video with real or fake label equals to giving the bag-level label. A fake video means that at least one face in this video has been manipulated.

In fact, even the state-of-the-art face forgery method like DeepFake \cite{DeepFakes} usually tampers the video by single-frame, which may cause some jitter in the nearby frames. But existing single-frame level methods are not sensitive enough to these jitters, which wastes a vital clue of fake video.


with multiple instances. In a multiple instance learning (MIL) task,


On the contrary, our MIL approach only requires a real or fake label for the video, which is much more convenient. 

In this paper, we introduce a novel problem of multi-instance face forgery detection and propose a novel network named Sharp Multi-Instance Learning Net (S-MIL Net) driven by a weighting mechanism. We design the network as a multi-scale architecture composed of a spatial-level encoding part and a temporal-level encoding part, which can learn local frame feature and nearby frame features, respectively. Given a video sequence, our approach can predict real or fake by considering the semantics among nearby frames rather than the max or mean score of several frames, which is more sensitive to the jitter. On the other hand, the proposed weighting mechanism relieves the vanishing gradients issue which commonly appears in the Multi-Instance learning task. In an MIL task, the key problem is the learning process from instance decision to bag level decision. The traditional method achieve the bag level decision without focus, which may cause gradients vanishing during the training. In our approach, the weighting mechanism is utilized to enhance the weights of important frames while weaken the irrelevant ones, which visually makes the gradient surface much sharper. 

Besides, we propose a new dataset named FaceForensics Plus with Mixing samples (FFPMS) for multi-instance detection, which only requires video-level label. We believe that this dataset can inspire more video-level methods and push the forgery detection field to a new level. Experiments on our FFPMS dataset verify that our approach is superior to other counterparts for multi-instance face forgery detection. Also, the proposed method can make a more accurate judge on whether a video is fake or not than other methods on DFDC benchmark. Moreover, our S-MIL Net can also be adapted to traditional single-frame detection task and achieves state-of-the-art performance on the FF++ datasets \cite{Faceforensics++}, showing a promising result for face information protection. 



The major contributions of our paper include: 

\begin{itemize}
\item We introduce a novel framework for multi-instance face forgery detection and a new FFPMS dataset with video-level annotation, which is more close to the practical application.

\item We propose a multi-scale network named S-MIL Net driven by a weighting mechanism, which can learn semantics among nearby frames and relieve the vanishing gradients issue as well.

\item We verify that our approach is superior to other counterparts for multi-instance face forgery detection and our S-MIL Net can also be adapted to traditional single-frame detection.
\end{itemize}

